An embedded genus-one helicoid

There exists a properly embedded minimal surface of genus one with one end. The end is asymptotic to the end of the helicoid. This genus one helicoid is constructed as the limit of a continuous one-parameter family of screw-motion invariant minimal surfaces--also asymptotic to the helicoid--that have genus equal to one in the quotient.

==> figures/figs_inc.tex <==

\def\begfig {
\begin{figure}
\small
}
\def\endfig {
\normalsize
\end{figure}
}

\newcommand{\path}{./figures/}

\def\h_one_rhombus {
\begfig
\hspace{0.3in} 
\epsfxsize = 3.0in 
\epsffile{\path fig1.eps} 
\hfill 
\begin{center} 
%\mbox Figure~1
\vspace{0.5cm}
\parbox{4.0in}{\caption{The rhombus model for the underlying Riemann surface 
of 
the quotient surface of \Hone/ modulo translations is drawn on the
left. The vertical points, $V_i$ and the horizontal points, $E_i$, on the
horizontal diagonal are included. The cycles $\alpha$ and $B$, illustrated 
on the right,
 and their reflections in
the vertical diagonal, generate a homology basis for the
punctured torus. 
}}
\end{center} 
\endfig
\label{h_one_rhombus}
}

\def\FigTwo {
\begfig
\hspace{0.3in} 
\epsfxsize = 3.0in 
\epsffile{\path fig2.eps} 
\hfill 
\begin{center} 
\mbox Figure~2
\vspace{0.5cm}
\parbox{2in}{
caption text here 2
}
\end{center} 
\endfig
}

\def\FigThree {
\begfig
\hspace{0.4in} 
\epsfxsize = 3.0in 
\epsffile{\path fig3.eps} 
\hfill 
\begin{center} 
\mbox Figure~3
\vspace{0.5cm}
\parbox{2in}{
caption text here 3
}
\end{center} 
\endfig
}

\def\FigFour {
\begfig
\hspace{0.9in} 
\epsfxsize = 1.9in 
\epsffile{\path fig4.eps} 
\hfill 
\begin{center} 
\mbox Figure~4
\vspace{0.5cm}
\parbox{2in}{
caption text here 4
}
\end{center} 
\endfig
}

\def\FigFive {
\begfig
\hspace{0.0in} 
\epsfxsize = 3.2in 
\epsffile{\path fig5.eps} 
\hfill 
\begin{center} 
\mbox Figure~5
\vspace{0.5cm}
\parbox{2in}{
caption text here 5
}
\end{center} 
\endfig
}

\def\FigSix {
\begfig
\hspace{0.4in} 
\epsfxsize = 3.0in 
\epsffile{\path fig6.eps} 
\hfill 
\begin{center} 
\mbox Figure~6
\vspace{0.5cm}
\parbox{2in}{
caption text here 6
}
\end{center} 
\endfig
}

\def\FigSeven {
\begfig
\hspace{0.2in} 
\epsfxsize = 3.3in 
\epsffile{\path fig7.eps} 
\hfill 
\begin{center} 
\mbox Figure~7
\vspace{0.5cm}
\parbox{2in}{
caption text here 7
}
\end{center} 
\endfig
}

\def\FigEight {
\begfig
\hspace{0.3in} 
\epsfxsize = 3.0in 
\epsffile{\path fig8.eps} 
\hfill 
\begin{center} 
\mbox Figure~8
\vspace{0.5cm}
\parbox{2in}{
caption text here 8
}
\end{center} 
\endfig
}

\def\FigNine {
\begfig
\hspace{0.0in} 
\epsfxsize = 3.7in 
\epsffile{\path fig9.eps} 
\hfill 
\begin{center} 
\mbox Figure~9
\vspace{0.5cm}
\parbox{2in}{
caption text here 9
}
\end{center} 
\endfig
}


